Canonical Proof Nets for Intuitionistic Multiplicative Linear Logic

We study the problem of finding canonical representations of proofs in the multiplicative fragment of intuitionistic linear logic with units. We show that, contrary to the classical case, it is possible to define a notion of proof nets for this fragment which is provided with a polynomial-time sequentialization procedure and is both canonical and efficient. In particular, we show that sequent calculus derivations differing only by a permutation of independent rule applications are translated to the same proof net, and that the translations between sequent calculus and proof nets are inverse to each other.

==> macros.tex <==
\newif\iftodo\todofalse
\usepackage{marginnote}
\usepackage{xargs} % needed for \newcommandx

\makeatletter
\newcommandx{\commenter}[3][2=red,3=]{%
  % #1 = long name
  % #2 = color (optional, default red)
  % #3 = short name (optional, defaults to #1)
  % --- define \<name>comment ---
  \expandafter\newcommand\csname #1\endcsname[1]{%
    {\color{#2}{#1: ##1}}\todotrue%
  }%
  % --- define \<name>cor ---
  \expandafter\newcommand\csname \if\relax\detokenize{#3}\relax#1\else#3\fi cor\endcsname[2]{%
    {\color{gray}{##1}}{\color{#2}{##2}}\todotrue%
  }%
  % --- define \<name> (margin short form) ---
  \expandafter\newcommand\csname m#1\endcsname[1]{%
    \marginpar{{\color{#2}$[\![$ ##1$]\!]$}}\todotrue%
  }%
}

\makeatletter

\commenter{todo}[red]
\commenter{tofix}[red]
\commenter{tocheck}[red]

\newcommand{\typocheck}[2]{{\color{red}#1}{\color{blue}#2}}

\newcommand{\ap}[1]{\textcolor{red}{\textbf{Action point:} #1}}




\def\variance{variance\xspace}
\def\test{test\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%
%		math symbols
%%%%%%%%%%%%%%%%%%%%%%%%

\def\set#1{\{#1\}}
\def\Set#1{\begin{Bmatrix}{#1}\end{Bmatrix}}
\def\SET#1#2{\left\{\begin{array}{l|l}#1&\begin{array}{l}#2\end{array}\end{array}\right\}}
\def\sizeof#1{|#1|}
\def\tuple#1{\langle#1\rangle}
\def\Tuple#1{\left\langle#1\right\rangle}

\newcommand{\intset}[2]{\set{#1, \dots, #2}}

\def\restr#1{|_{#1}}
\def\hider{\mathsf{hide}}

\def\giso{\equiv}
\def\feq{\equiv}
\def\gsim{\approx}

\def\dD{\mathcal{D}}

%%%%%%%%%%%%%%%%%%%%%%%%
%		proof nets
%%%%%%%%%%%%%%%%%%%%%%%%

\def\nonefo{\none_{\mathrm{forgo}}}
\def\nonefa{\none_{\mathrm{faith}}}


\def\ps{\mathsf{S}}
\def\pn{\mathsf{P}}
\def\pnp{\pn'}



\def\nodeset{\mathsf N}
\def\gateset{\mathsf G}
\def\gate{\mathfrak g}


\pzedges{F}{draw=lightgray,>=stealth,->}{}
\pzedges{PATH}{>=stealth,->,draw=pzgreen}{}
\pzedges{RPATH}{>=stealth,->,draw=red}{}
\pzedges{AF}{draw=gray}{}



\def\cC{\bclr{\mathcal C}}

\def\sizeofaof{|\aof|_{+\lone\text s}}

\def\cutelim{\rightsquigarrow_{\cutr}}
\def\cutelims{\cutelim^*}
\def\vcutelim{\rotatebox{-90}{$\rightsquigarrow$}_{\cutr}}

\def\an{{\bclr{\mathcal N}}}
\def\as{{\bclr{\mathcal S}}}

%%%%%%%%%%%%%%%%%%%%%%%%
%	Logic Formulas
%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\proves}[1][]{\mathord{\vdash_{#1}\,}}



%% Math standard symbols
\def\N{\mathbb N}
\def\formulas{\mathcal F}
\def\atoms{\mathbb A}
\def\labSet{\mathbb L}

\def\chole{\cdot}
\newcommand{\ctx}[1][\chole]{{[{#1}]}}
\newcommand{\Ctx}[1]{{\left[{#1}\right]}}




\usepackage{bbold}
\def\lone{{\mathbb 1}}
\def\none{\cneg\lone}
\def\ntens{\mathop{\cneg{\ltens}}}
\def\nimp{\mathop{\cneg\limp}}




\def\isw#1{#1^\circ}
\def\isb#1{#1^\bullet}
\def\npar{\lpar^\bullet}
\def\ppar{\lpar^\circ}




%%%%%%%%%%%%%%%%%%%
%%Graphs
%%%%%%%%%%%%%%%%%%%
\def\labSet{\mathcal L}


\newcommand\rclr[1]{{\color{red}#1}}
\newcommand\gclr[1]{{\color{blue}#1}}
\newcommand\bclr[1]{{\color{blue}#1}}
\newcommand\aclr[1]{{\color{pzbrickred}#1}}
\newcommand\mclr[1]{{\color{pzgreen}#1}}
\newcommand\sclr[1]{{\color{skewcolor}#1}}

\def\gG{\mathcal G}
\def\gH{\mathcal H}
\def\gF{\mathcal F}
\def\gJ{\mathcal J}
\def\gK{\mathcal K}
\def\gI{\mathcal I}
\def\gP{\mathcal P}

\newcommand{\cgF}{{\gclr\gF}}
\newcommand{\cgG}{{\gclr\gG}}
\newcommand{\cgH}{{\gclr\gH}}
\newcommand{\cgK}{{\gclr\gK}}
\newcommand{\cgJ}{{\gclr\gJ}}
\newcommand{\cgI}{{\gclr\gI}}

\def\ar{\mathcal A}
\newcommand{\lab}[1][]{\ell_{#1}}
\newcommand{\labof}[2][]{\ell_{#1}(#2)}

\newcommand{\arof}[1]{{\llbracket#1\rrbracket}}
\newcommand{\emptyar}{{\color{pzbrickred}\emptyset}}
\newcommand{\emptycutof}{{\bclr{\emptyset}}}
\newcommand{\treeof}[1]{\mathsf{tree}(#1)}
\newcommand{\emptylink}{{\color{linkcolor}\emptyset}}

\def\path{\mathfrak p}

%%%%%% Rules symbols
\def\axrule{\mathsf{ax}}
\def\AXrule{\mathsf{AX}}
\def\cutr{\mathsf{cut}}
\def\mixr{\mathsf{mix}}
\def\llimp{\mathsf{\nimp}}
\def\rlimp{\mathsf{\limp}}
\def\lltens{\mathsf{\ntens}}
\def\rltens{\mathsf{\ltens}}
\def\loner{\lone}
\def\lonel{\none}

\def\Crule{\mathsf C}
\def\Wrule{\mathsf W}

\def\IMLL{\mathsf{IMLL}}
\def\IMLLm{\mathsf{IMLL}^-}
\def\MLL{\mathsf{MLL}}
\def\MALL{\mathsf{MALL}}
\def\MELL{\mathsf{MELL}}
\def\IMELL{\mathsf{IMELL}}
\def\pIMLL{\IMLL^{\intsym}}
\def\LJ{\mathsf{LJ}}

\def\gsum{+}
\def\gimp{{\aclr-\hspace{-2pt}\lcoseq}}

% \newcommand{\axlink}[1][]{\mkern1mu\mathord{\stackrel{#1}{{\gclr\rightharpoonup}}}\mkern1mu}
% \newcommand{\axeq}[1][]{\mkern1mu\mathord{\stackrel{#1}{{\gclr\sqcap}}}\mkern1mu}
% \newcommand{\aedge}[1][]{\mkern1mu\mathord{\stackrel{#1}{{\color{pzbrickred}\rightarrow}}}\mkern1mu}
\newcommand{\cutarrow}{%
  \mathrel{%
    \tikz[baseline=-2.5pt]{
    \draw[bend left=30,thick] (0,0) to (2ex,0);
    \draw[thick] (2ex,0) circle (0.12em);
    \fill (2ex,0) circle (0.12em);
    }%
  }%
}
\newcommand{\axarrow}{%
  \mathrel{%
    \tikz[baseline=-2.5pt]{
      \draw[bend left=30,thick] (0,0) to (2ex,0);
      \draw[thick] (2ex,0) circle (0.12em);
	    \fill[white] (2ex,0) circle (0.10em);
    }%
  }%
}
% \def\cutarrow{\rightharpoonup}
% \def\axarrow{\rightharpoondown}


\newcommand{\singlevertex}[1][]{\bullet_{#1}}

\newcommand{\vof}[1][]{V_{#1}}
\newcommand{\vuof}[1][]{V_{#1}^\lone}
\newcommand{\vaof}[1][]{V_{#1}^\atoms}
\newcommand{\dof}[1][]{\mkern1mu{{\to}_{#1}}\mkern1mu}
\newcommand{\eof}[1][]{\mkern1mu{\aclr{\to}_{#1}}\mkern1mu}
\newcommand{\Eof}[1][]{\mkern1mu{{\to}_{#1}}\mkern1mu}
\newcommand{\jof}[1][]{\mkern1mu{{\to^j}_{#1}}\mkern1mu}
\newcommand{\hof}[1][]{\mkern1mu{{\bclr{\to}}_{#1}}\mkern1mu}
\newcommand{\oof}[1][]{\mkern1mu{\aclr{\to}^\bullet_{#1}}\mkern1mu}
\newcommand{\ueof}[1][]{\mkern1mu{^\lone\aclr{\to}^\circ_{#1}}\mkern1mu}
\newcommand{\coof}[1][]{\mkern1mu{\aclr{\mapsto}^\bullet_{#1}}\mkern1mu}
\newcommand{\aof}[1][]{\mkern1mu{\gclr{\gclr{\axarrow}}_{#1}}\mkern1mu}
\newcommand{\cutof}[1][]{\mkern1mu{\gclr{\gclr{\cutarrow}}_{#1}}\mkern1mu}

\def\Den#1{\begin{Bmatrix}\!\!\begin{Bmatrix}#1\end{Bmatrix}\!\!\end{Bmatrix}}
\def\trans#1{\bclr{\Den{\color{black}#1}}}
\def\jtrans#1{\bclr{\Den{\color{black}#1}^j}}
\def\enof#1{\Den{#1}^e}
\def\pnof#1{\left\llbracket#1\right\rrbracket}
\def\cpnof#1{\left\llbracket#1\right\rrbracket^{\mathsf{max}}}

\def\link{\bclr{\lambda}}
\newcommand{\links}[1][]{\bclr{\Lambda}_{#1}}
\def\depends{\prec}
\def\independs{\;\|\;}

\def\redsetname{residual set\xspace}
\def\redset#1{\mathsf{Res}_{#1}}

\def\linkgraph#1{\overrightarrow{#1}}
\def\linkcutgraph#1{\widetilde{#1}}

\newcommand{\rootsof}[1][]{{\mathfrak R}_{#1}}
% \newcommand{\isrof}[1][]{\rootof{#1}}
% \def\drootof#1{{\not\!\!\dof}_{#1}}
% \newcommand{\isdrof}[1][]{\drootof{#1}}


\pzvertex{hid}{~}{}
\newcommand{\aedge}[2][1.5em]{
	\vhid1 
	\hskip#1
	\vhid2
	\Aledges{hid1/hid2/#2}
}
% \newcommand{\axlink}[1][]{\mkern1mu\mathord{\stackrel{#1}{{\gclr\rightharpoonup}}}\mkern1mu}


% %%%%%%%%%%%%%%%%%%%%%
% % 		games
% %%%%%%%%%%%%%%%%%%%%%

% \def\strat{\mathcal S}
% \def\ttrat{\mathcal T}
% \def\rtrat{\mathcal R}


% \def\intsym{{\raisebox{1pt}{\resizebox{4pt}{!}{\rotatebox[origin=c]{180}{\LEFTcircle}}}}}
% \def\tnisym{{\raisebox{1pt}{\resizebox{4pt}{!}{\rotatebox[origin=c]{0}{\LEFTcircle}}}}}
% \def\isbw#1{#1^\intsym}
% \def\iswb#1{#1^\tnisym}

% \def\upsym{{\raisebox{1.2pt}{\resizebox{3.5pt}{!}{\rotatebox[origin=c]{90}{\LEFTcircle}}}}}
% \def\dnsym{{\raisebox{1.2pt}{\resizebox{3.5pt}{!}{\rotatebox[origin=c]{-90}{\LEFTcircle}}}}}

% \def\diasym{{\raisebox{1.2pt}{\resizebox{5pt}{!}{\rotatebox[origin=c]{45}{\LEFTcircle}}}}}
% \def\aidsym{{\raisebox{1.2pt}{\resizebox{5pt}{!}{\rotatebox[origin=c]{225}{\LEFTcircle}}}}}

% \def\inter#1#2#3{#1\overset{#3}\intsym#2}
% \def\comp#1#2#3{#1\overset{#3}\ast#2}
% \def\flip#1{\mathsf{flip}(#1)}
% \def\doubleflip#1{\overline{\overline{#1}}}

%%%%%%%%%%%%%%%%%%%%%
% 		Math acronyms
%%%%%%%%%%%%%%%%%%%%%


\def\mathacronym{\mathsf}

\def\dagmacro{$\mathacronym{dag}$}
\def\mamacro{$\mathacronym{MA}$}
\def\ddagmacro{$\operatorname{2-\mathacronym{dag}}$}

\def\smcc{\textsf{SMCC}\xspace}
\def\smccs{\textsf{SMCC}s\xspace}

\def\ma{\mamacro\xspace}
\def\mas{\mamacro s\xspace}

\def\dag{\dagmacro\xspace}
\def\dags{\dagmacro s\xspace}

\def\comPspace{\textbf{PSPACE}}
\def\comPtime{\textbf{PTIME}}




%%%%%%%%%%%%%%%%%%%%%
% 		Formatting
%%%%%%%%%%%%%%%%%%%%%
\providecommand{\myparagraph}[1]{\textbf{#1}. }
\def\defn#1{\textbf{#1}}
\def\IH{\text{ Ind. Hyp.}}


\def\quand{\quad\mbox{and}\quad}
\def\qquand{\qquad\mbox{and}\qquad}
\def\qomma{\; , \;}
\def\qqomma{\quad , \quad}
\def\qdot{\quad\mbox{.}}

\def\quor{\quad\mbox{or}\quad}

\def\resp#1{(resp. #1)}







%%%%%%%%%%%%%%%%%%%%%
% 		equivalences 
%%%%%%%%%%%%%%%%%%%%%
\def\preq{\sim}
\def\preqq{\approx}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\prenet#1#2{{\bclr{#1}}:: #2}
\def\genpren{\prenet{\links}{\Gamma\vdash A}}%
\def\genprenp{\prenet{\links'}{\Gamma\vdash A}}%
\def\testof#1{\mathcal T(#1)}%
\pzvertex{ntens}{\ntens}{}%
\pzvertex{nimp}{\nimp}{}%
\pzvertex{none}{\none}{}%
\def\pathto{\to\!\!\!\!\!\to}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def\testof#1{\mathcal{T}(#1)}
\def\nr{\mathfrak r}
\def\nn{\mathfrak n}
\def\nodeof#1{\nn_{#1}}

\def\wone{\isw \lone}
\def\bone{\isb \lbot}

\def\intsym{{\raisebox{1pt}{\resizebox{4pt}{!}{\rotatebox[origin=c]{90}{\LEFTcircle}}}}}
\def\tnisym{{\raisebox{1pt}{\resizebox{4pt}{!}{\rotatebox[origin=c]{270}{\LEFTcircle}}}}}
\def\isbw#1{#1^\intsym}
\def\iswb#1{#1^\tnisym}

\def\wtens{\isw\ltens}
\def\btens{\isb\ltens}
\def\wpar{\isw\lpar}
\def\bpar{\isb\lpar}


\pzedges{H}{draw=yellow,line width=5pt,line cap=round,opacity=0.5}{}
\pzedges{GOOD}{draw=green,line width=5pt,line cap=round,opacity=0.5}{}
\pzedges{BAD}{draw=red,line width=5pt,line cap=round,opacity=0.5}{}
\pzedges{dashUA}{draw=pzbrickred,dashed}{}







\newcommand{\nodn}[4]{\vlinf{#2}{#4}{#3}{#1}}
\newcommand{\nodt}[4]{\vlidf{#2}{#4}{#3}{#1}}
\def\wrule{\!\!\circ}
\def\brule{\!\!\bullet}
\def\isw#1{{#1}^\circ}
\def\isb#1{{#1}^\bullet}
\def\isu#1{{#1}^\ast}




\def\airule{\mathsf{ai}}
\def\irule{\mathsf{i}}
\def\swir{\mathsf{s}}
\def\comrule{\mathsf{com}}
\def\assorule{\mathsf{asso}}
\def\curryrule{\mathsf{cur}}

\def\curry{\mathsf{cur}}
\def\uncurry{\mathsf{ruc}}


\def\waidr{\mathsf{ai}_\downarrow^\circ}
\def\baidr{\mathsf{ai}_\downarrow^\bullet}
\def\baiur{\mathsf{ai}_\uparrow^\bullet}

% \def\tudr{\mathsf{u}_\downarrow^{\ltens}}
% \def\ludr{\mathsf{u}_\downarrow^{\limp}}
% \def\tuur{\mathsf{u}_\uparrow^{\ltens}}
% \def\luur{\mathsf{u}_\uparrow^{\limp}}

\def\tassr{\mathsf{asso}^{\ltens}}

\def\wlsr{\mathsf{s_L^\circ}}
\def\wtsr{\mathsf{s_R^\circ}}
\def\blsr{\mathsf{s_L^\bullet}}
\def\btsr{\mathsf{s_R^\bullet}}

\def\tcomr{\comrule^{\ltens}}
